Pure Pattern Calculus \`a la de Bruijn

It is well-known in the field of programming languages that dealing with variable names and binders may lead to conflicts such as undesired captures when implementing interpreters or compilers. This situation has been overcome by resorting to de Bruijn indices for calculi where binders capture only one variable name, like the $\lambda$-calculus. The advantage of this approach relies on the fact that so-called $\alpha$-equivalence becomes syntactical equality when working with indices. In recent years pattern calculi have gained considerable attention given their expressiveness. They turn out to be notoriously convenient to study the foundations of modern functional programming languages modeling features like pattern matching, path polymorphism, pattern polymorphism, etc. However, the literature falls short when it comes to dealing with $\alpha$-conversion and binders capturing simultaneously several variable names. Such is the case of the Pure Pattern Calculus (PPC): a natural extension of $\lambda$-calculus that allows to abstract virtually any term. This paper extends de Bruijn's ideas to properly overcome the multi-binding problem by introducing a novel presentation of PPC with bidimensional indices, in an effort to implement a prototype for a typed functional programming language based on PPC that captures path polymorphism.

==> proofs/upd-properties.tex <==
\begin{lemma}[Commutativity of $\updvv$ and $\updmm$] Let $l,k\in\NN$ and $t\in\termPPCX$, then the following properties hold
\label{lema-upd-commutativity}
\begin{enumerate}
\item  \label{updv-updm} $\updv[k]{\updm[l]{t}} = \updm[l]{\updv[k]{t}}$
\item If $k > l$
  \begin{enumerate}
  \item \label{updv-updv} $\updv[k]{\updv[l]{t}} = \updv[l]{\updv[k-1]{t}}$
  \item \label{updm-updm} $\updm[k]{\updm[l]{t}} = \updm[l]{\updm[k-1]{t}}$
  \end{enumerate}
\end{enumerate}
\end{lemma}
\begin{proof} Easy induction on $t$.
\end{proof}
\alexis{lo puse para una versión de una demo, pero esa versión no quedó. así que este lema no sé si hace falta.}

\begin{lemma}[Inversibility of $\updvv$]
\label{lema-updv-plusminus-inversion}
  For $k\in\NN$ and $t\in\termPPCX$
  \begin{enumerate}
  \item \label{minus-vs-plus} $\updvneg[k]{\updv[k]{t}} = t$
  \item \label{k+1-notin-pi1} $k+1\notin\pi_1(\FV(\updv[k]{t}))$
  \item \label{plus-vs-minus} $\updv[k]{\updvneg[k]{t}} = t \iff k+1\notin\pi_1(\FV(t))$
  \end{enumerate}
\end{lemma}
\begin{proof} Easy induction on $t$.
\end{proof}
